Multi-Fidelity Methods for Optimization: A Survey

Real-world black-box optimization often involves time-consuming or costly experiments and simulations. Multi-fidelity optimization (MFO) stands out as a cost-effective strategy that balances high-fidelity accuracy with computational efficiency through a hierarchical fidelity approach. This survey presents a systematic exploration of MFO, underpinned by a novel text mining framework based on a pre-trained language model. We delve deep into the foundational principles and methodologies of MFO, focusing on three core components -- multi-fidelity surrogate models, fidelity management strategies, and optimization techniques. Additionally, this survey highlights the diverse applications of MFO across several key domains, including machine learning, engineering design optimization, and scientific discovery, showcasing the adaptability and effectiveness of MFO in tackling complex computational challenges. Furthermore, we also envision several emerging challenges and prospects in the MFO landscape, spanning scalability, the composition of lower fidelities, and the integration of human-in-the-loop approaches at the algorithmic level. We also address critical issues related to benchmarking and the advancement of open science within the MFO community. Overall, this survey aims to catalyze further research and foster collaborations in MFO, setting the stage for future innovations and breakthroughs in the field.

==> makefile <==
FILE=main

all:	
	latex $(FILE)
	bibtex $(FILE)
	latex $(FILE)
	latex $(FILE)
	dvips -o $(FILE).ps $(FILE).dvi
	ps2pdf $(FILE).ps
	open $(FILE).pdf

clean:
	rm -f *.aux *.blg *.log *.bbl *.out *.bak *.synctex.gz *.synctex.gz\(busy\) *.tex~

cleanall: clean
	rm -f *.dvi $(FILE).ps $(FILE).pdf


==> method.tex <==
%!TeX root=main.tex

\section{Proposed Method}
\label{sec:method}

\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figs/workflow.pdf}
    \caption{Flowchart of \our. It iterates between the \texttt{preference elicitation} and the \texttt{policy optimization} modules until the stopping criterion is met, and outputs the preferred policies.}
    \label{fig:flowchart}
\end{figure*}

\pref{fig:flowchart} presents the modular flow chart of our proposed \our\ framework. It consists of three core modules: $i$) the \texttt{seeding} module that obtains a set of promising seeding policies; $ii$) the \texttt{preference elicitation} module that plays as the interface where the DM interacts with the MORL and it learns the DM's preference from her feedback; and $iii$) the \texttt{policy optimization} module that leverages the learned preference to guide the search for the policy of interest. Note that the last two modules iterate between each other until the stopping criterion is met. In the following paragraphs, the implementation of each module is delineated step by step.

\subsection{Seeding Promising Policies}
\label{sec:seeding}

The \texttt{seeding} module operates as a conventional MORL, disregarding the DM's preference information and instead searching for a set of trade-off policies that approximate the PF. In this paper, our fundamental approach for MORL is inspired by the prevalent multi-objective evolutionary algorithm based on decomposition (MOEA/D)~\cite{ZhangL07,ChenL23}. We propose decomposing the MORL problem into a collection of subproblems, each representing a linear aggregation of different objective functions:
\begin{equation}
    \tilde{J}(\pi,\mathbf{w})=\sum_{i=1}^mw_iJ_{i}(\pi),
    \label{eq:ws}
\end{equation}
where $\mathbf{w}=(w_1,\ldots,w_m)^\top$ and $\sum_{i=1}^mw_i=1$ is the weight vector that represents certain preferences for different objectives. Note that any aggregation function can be applied in the \our\ framework, while we will investigate this aspect in~\pref{sec:rq6} of our empirical study. To balance convergence and diversity, we employ the Das and Dennis' method~\cite{DasD98} to define a set of weight vectors $\mathcal{W}=\{\mathbf{w}^i\}_{i=1}^N$ evenly distributed along a unit simplex. Here, $N=$ ${H+m-1}\choose{m-1}$, and $H>1$ is the number of equally spaced divisions along each coordinate.%\footnote{The Das and Dennis' method is further explained in Section 2.1 of the supplemental document.}.

In the \our\ framework, all subproblems are handled simultaneously in a parallel manner, with each treated as an individual RL task. It is important to note that each RL policy is associated with a dedicated weight vector (i.e., a subproblem) in our \our\ framework. Given the continuous state and action spaces of the RL tasks considered in this paper, we employ proximal policy optimization (PPO)~\cite{SchulmanWDRK17}, a policy-gradient algorithm that optimizes the policy by explicitly updating the policy network $\pi_\theta$ using a gradient-based method. The objective function of the PPO is:
\begin{equation}
    \begin{aligned}
        J^{\mathrm{clip}}(\pi_\theta)=&\mathbb{E}_t\bigg[\min\bigg(\frac{\pi_{\theta}(a_t|s_t)}{\pi_{\theta_{\mathrm{old}}}(a_t|s_t)}\hat{A}_t,\\& \mathrm{clip}\left(\frac{\pi_{\theta}(a_t|s_t)}{\pi_{\theta_{\mathrm{old}}}(a_t|s_t)},1-\epsilon,1+\epsilon\right)\hat{A}_t\bigg)\bigg],
    \end{aligned}
    \label{eq:ppo}
\end{equation}
where $\hat{A}_t$ is an advantage function that estimates the performance of the current state-action tuple $\langle s_t,a_t\rangle$, and $\epsilon\in\left(0,1\right)$ controls the range of policy updates to avoid excessive optimization. The pseudo code of this multi-objective PPO (\texttt{MOPPO}) is given in~\pref{alg:moppo}, the output of which is the set of non-dominated policies, denoted as $\Pi$.

\begin{remark}
    The motivation of this \texttt{seeding} module stems from our preliminary experiments, which showed that interacting with the DM and conducting preference learning at the beginning of \our\ is ineffective. This observation can be attributed to the fact that the initial trade-off policies are far from the PF, which can be misleading for the DM during preference elicitation. As a result, we introduce the \texttt{seeding} module to first search for a set of reasonably good trade-off policies before proceeding with preference learning. This approach aims to provide a better starting point for the subsequent steps in the \our\ framework.
\end{remark}

\begin{algorithm}[t!]
    \caption{\texttt{MOPPO}}
    \label{alg:moppo}
    \KwIn{$t_\mathrm{r}$: \# of environment steps, $\overline{\Pi}$: stored policies}
  	Initialize $\Pi:=\emptyset$ for storing optimized policies\;
	\ForEach{$\langle\pi^i,\mathbf{w}^i\rangle\in\overline{\Pi}$}{\tcc{every task works parallelly}
        \While{the stopping criterion is not met}{
            Execute $\pi^i$ and store the collected trajectory data in a buffer $\mathcal{S}^i:=\left(\langle s^i_1,a^i_1,r^i_1\rangle,\ldots,\langle s^i_{t_\mathrm{r}},a^i_{t_\mathrm{r}},r^i_{t_\mathrm{r}}\rangle\right)$\;
            \While{the stopping criterion is not met}
            {
                Sample a trajectory from $\mathcal{S}^i$, and use $\mathbf{w}^i$ to aggregate its rewards\;
                Calculate $\mathcal{\hat{A}}_t$ as mentioned in~\cite{SchulmanMLJA15}\;
                Update $\pi^i$ by optimizing $J^{\mathrm{clip}}(\pi^i)$ in~\pref{eq:ppo}\;
            }
            Insert updated task $\langle\pi^i,\mathbf{w}^i\rangle$ to $\Pi$\;
        }
    }
    \Return Non-dominated policies in $\Pi$
\end{algorithm}

\subsection{Preference Elicitation}
\label{sec:preference_elicitation}

This module is the crux of proposed \our, whose pseudo code is given in~\pref{alg:pl}. It consists of three steps including \texttt{consultation}, \texttt{preference learning}, and \texttt{preference translation}. They are designed to address the following three questions. %$i$) how to collect the DM's feedback; $ii$) how to model the DM's preference information; and $iii$) how to leverage the learned preference information to guide MORL.
%The pseudo code of this \texttt{preference elicitation} process is given in~\pref{alg:pl}, and more detailed information can be found in~\cite{ChuG05}.

\subsubsection{How to collect the DM's feedback}
\label{sec:interaction}

In the \texttt{preference elicitation} module, the \texttt{consultation} step serves as an interface where the DM is asked to provide feedback on the quality of selected policies based on their preferences. In this work, we consider an indirect preference information in the form of holistic pairwise comparisons of policy pairs $\langle\pi^1,\pi^2\rangle$. The outcome of this pairwise comparison can be $\pi^1$ being \textit{better}, \textit{worse}, or \textit{indifferent} compared to $\pi^2$, denoted as $\pi^1\succ\pi^2$, $\pi^1\prec\pi^2$, or $\pi^1\simeq\pi^2$, respectively. Asking the DM to compare all ${|\Pi|}\choose{2}$ policy pairs derived from the seeding policies obtained in the \texttt{seeding} module may overwhelm them. To alleviate this issue, we only choose the two most informative policies from $\Pi$ to consult the DM. Our preliminary experiments showed that this approach not only significantly reduces the DM's workload but is also sufficient for preference learning in \our. Inspired by~\cite{Auer02}, we evaluate the information of a policy $\pi\in\Pi$ as:
\begin{equation}
    \mathtt{I}(\pi)=\mu(\pi)+\alpha\sqrt{{\sigma(\pi)\tilde{n}}/{\tilde{n}_\pi}},
    \label{eq:information}
\end{equation}
where $\mu(\pi)$ and $\sigma(\pi)$ represent the mean and variance predicted by the preference model, which will be introduced in~\pref{sec:preference_model}. $\tilde{n}_\pi$ denotes the number of times $\pi$ has been queried in previous interactions, $\tilde{n}$ represents the total number of queries incurred so far, and $\alpha>0$ is a parameter that balances exploitation and exploration. Based on this definition, two policies $\pi^1=\argmax_{\pi\in\Pi}\mathtt{I}(\pi)$ and $\pi^2=\argmax_{\pi\in\Pi\setminus{{\pi^1}}}\mathtt{I}(\pi)$ are chosen for the \texttt{consultation} step. The queried policies are stored in a dedicated set $\tilde{\Pi}$.

\begin{remark}
    In principle, we can employ \texttt{MOPPO}, as in the \texttt{seeding} module, to obtain a set of policies that approximate the entire PF. However, these non-dominated policies may be too diverse for DMs to identify their preferred ones that satisfy their aspirations in practice. Thus, a more refined approach is required to accommodate the DM's specific preferences.
    %In principle, we can directly go with multi-objective PPO as in the \texttt{seeding} module to obtain a set of policies that approximate the entire PF. However, these non-dominated policies can be too diverse for the DMs to identity their preferred ones satisfying their aspirations in practice.
\end{remark}

\begin{remark}

    At the beginning of the \texttt{preference elicitation} module, no data has been collected from the DM to train the preference model. To address this, during the first $\tau > 1$ iterations, we randomly select two policies in the \texttt{consultation} step. This approach allows us to gather initial data and subsequently refine the preference model as more information becomes available.
\end{remark}

\begin{remark}
    In the context of MORL, the DM's preference can be represented by assigning weights to different objective functions based on their importance~\cite{WrayZM15,NatarajanT05,YangSN19,WirthFN16}. However, this presents a paradox in our context, as the preference is unknown a priori. An alternative approach is to assign a numeric score to each candidate~\cite{LiCSY19}. Nevertheless, as discussed in~\cite{ZintgrafRLJN18}, this method can be vague and challenging for non-domain experts to comprehend and apply effectively.
\end{remark}

\begin{remark}
    Note that the \texttt{preference elicitation} module in \our\ is highly efficient where we only need consult the DM once at each round with a pair of candidates.
\end{remark}

\subsubsection{How to model the DM's preference information}
\label{sec:preference_model}

Based on the holistic pairwise comparison(s) collected in the \texttt{consultation} step, the goal of the \texttt{preference learning} step is to learn a preference model that evaluates the quality of solutions according to the DM’s preference. Here our preference model is represented as a utility function $u(\pi):\mathbb{R}^m\rightarrow\mathbb{R}$ such that the ranking order of a set of testing policies $\hat{\Pi}$ satisfy that $\forall\pi^1,\pi^2\in\hat{\Pi}$, $u(\pi^1)>u(\pi^2)$ if $\pi^1\succ\pi^2$ and $u(\pi^1)=u(\pi^2)$ if $\pi^1\simeq\pi^2$. This paper applies a zero-mean Gaussian process (GP)~\cite{GPML} with the radial basis function kernel to serve as the regression model. In particular, $\tilde{\Pi}=\{\tilde{\pi}^i\}_{i=1}^\kappa$ is used as the training data where $\kappa$ is the number of policies queried at the \texttt{consultation} step. Then, we train $u(\pi)$ based on maximum a posterior estimation as:
\begin{equation}
    u^\star=\argmax\limits_u\mathbb{P}(u)\mathbb{P}(\tilde{\Pi}|u),
    \label{eq:map}
\end{equation}
where $\mathbb{P}(u)$ is a zero-mean Gaussian and $\mathbb{P}(\tilde{\Pi}|u)=\prod\limits_{i=1}^{\frac{\kappa}{2}}\Phi(\frac{u(\pi_i^1)-u(\pi_i^2)}{\sqrt{2}})$ is 
the likelihood of $u(\pi)$, $\Phi(\cdot)$ is the standard normal cumulative distribution. As in~\cite{ChuG05}, for each pair of $\left\langle{u(\pi_i^1),u(\pi_i^2)}\right\rangle$ where $\pi_i^1\succ\pi_i^2$, solving~\pref{eq:map} is equivalent to solving the following minimization problem: 
\begin{equation}
    \mathrm{minimize} -\sum\limits_{i=1}^{\frac{\kappa}{2}}\bigg{[}\Phi(\frac{u(\pi_i^1)-u(\pi_i^2)}{\sqrt{2}})+\frac{1}{2}u^{\top}(\pi_i^1)K^{-1}u(\pi_i^2)\bigg{]},
    \label{eq:minimize}
\end{equation}
where $K$ is the covariance matrix of $\tilde{\Pi}$. By 
applying Newton-Raphson formula, we can finally get the numerical approximation of the real $u^\star$. Given a testing policy $\pi^\star$, the mean and variance of $u^\star(\pi^\star)$ are predicted as 
$\mathrm{\mu}(\pi^\star)={\mathbf{k}^\star}^{\top}K^{-1}\mathbf{U}$ and 
$\mathrm{\sigma}(\pi^\star)=k(\pi^\star,\pi^\star)-{\mathbf{k}^\star}^{\top}(K+\Lambda^{-1})^{-1}{\mathbf{k}^\star}$, respectively, 
where $\mathbf{U}=(u^\star(\tilde{\pi}^1),\ldots,u^\star(\tilde{\pi}^\kappa))^\top$. $\mathbf{k}^\star$ is the covariance vector between $\tilde{\Pi}$ and $\pi^\star$. $\Lambda^{-1}$ is a $\kappa\times\kappa$ matrix for estimating $\mathbf{U}$.

\begin{algorithm}[t!]
    \caption{\texttt{preference elicitation}}
    \label{alg:pl}
    \KwIn{$\Pi$: stored non-dominated policies, $\tilde{\Pi}$: queried policies as training data, $u(\pi)$: preference model}% $\mathcal{W}$: weight vector set.}
    \tcc{consultation step}
    \eIf{random selection}{
        Randomly sample two policies $\pi^1$, $\pi^2$ from $\Pi$.
        }{
        \ForEach{$\pi\in\Pi$}{
        	Evaluate its utility value $u(\pi)$ and $\mathtt{I}(\pi)$\;}
        $\pi^1:=\argmax_{\pi\in\Pi}\mathtt{I}(\pi)$, $\pi^2:=\argmax_{\pi\in\Pi\setminus{\{\pi^1\}}}\mathtt{I}(\pi)$\;
        }
        Query the DM with $\pi^1$ and $\pi^2$, store the result in $\tilde{\Pi}$\;
        \tcc{preference learning step}
        Use the DM's feedback to update $\tilde{\Pi}$ and the preference model $u(\pi)$ as in~\pref{sec:preference_model}\;
        \tcc{preference translation step}
        Generate the new policy set $\Pi$ as in~\pref{sec:translation}\; 
        \Return $\Pi$, $\tilde{\Pi}$, $u(\pi)$.
\end{algorithm}

\subsubsection{How to leverage the learned preference information}
\label{sec:translation}

\begin{figure}[htbp]
    \centering
    \includegraphics[width=.85\linewidth]{flow/weight_adjustment.pdf}
    \caption{Illustration of the weight vector adjustment in Step 4. (a) The ROI is highlighted as the shaded cone region versus the evenly distributed weight vectors (denoted as $\newmoon$). (b) Adjusted weight vectors towards the ROI (denoted as \textcolor{blue}{$\newmoon$}).}
    \label{fig:preference_elicitation}
\end{figure}

In the \texttt{preference translation} step, the learned preference information is converted into a format that can be used to guide the \texttt{policy optimization} module. In the context of our proposed \our, this involves generating a new policy archive $\Pi$ for the next round of the policy optimization. This process consists of five steps:
\begin{enumerate}[Step 1:]
    \item Assign a preference score $\psi(\pi)=\mu(\pi)+\beta\sigma(\pi)$ to each policy $\pi\in\Pi$.
    \item Rank the policies in $\Pi$ based on the preference scores from Step 1. Identify the top $\kappa_1$ policies to construct a temporary policy archive $\dot{\Pi}$. Store the weight vectors associated with these policies, considered as promising, in a temporary archive $\dot{\mathcal{W}}=\{\dot{\mathbf{w}}^i\}_{i=1}^{\kappa_1}$.
    \item Generate a set of evenly distributed weight vectors $\tilde{\mathcal{W}}=\{\tilde{\mathbf{w}}^i\}_{i=1}^{\tilde{N}}$, as in the \texttt{seeding} module, where $\tilde{N}>N$. Set another temporary archive $\ddot{\mathcal{W}}=\emptyset$.
    \item Generate a set of weight vectors biased towards the region of interest (ROI), as illustrated in~\pref{fig:preference_elicitation}. Then, for $i=1$ to $\tilde{N}$, perform the following:
        \begin{enumerate}[Step 4.1:]
            \item Determine the reference point of $\tilde{\mathbf{w}}^i$ as $\mathbf{w}^\mathrm{r}=\argmin_{\dot{\mathbf{w}}\in\dot{\mathcal{W}}}|\dot{\mathbf{w}}-\tilde{\mathbf{w}}^i|$.
            \item Move $\tilde{\mathbf{w}}^i$ towards $\mathbf{w}^\mathrm{r}$ as $\ddot{w}^i_j=\tilde{w}^i_j+\eta(w^\mathrm{r}_j-\tilde{w}^i_j)$, where $j\in\{1,\cdots,m\}$.
            \item Update $\ddot{\mathcal{W}}$ with the new weight vector: $\ddot{\mathcal{W}}=\ddot{\mathcal{W}}\bigcup\{\ddot{\mathbf{w}}\}$ and return to Step 4.
        \end{enumerate}
    \item Randomly select $\kappa_2$ weight vectors from $\ddot{\mathcal{W}}$ and remove the others to form a reduced $\ddot{\mathcal{W}}$. Randomly choose $\kappa_2$ policies from $\dot{\Pi}$ and associate each selected policy with a weight vector in $\ddot{\mathcal{W}}$ to form a temporary archive $\ddot{\Pi}$. Construct the new policy archive $\Pi$ for the next round of the policy optimization as $\Pi=\dot{\Pi}\bigcup\ddot{\Pi}$.
\end{enumerate}

\begin{remark}
    In Step 1, $\psi(\pi)$ serves as an approximate value function that evaluates the satisfaction of policy $\pi$ concerning the DM's preference information. Notably, the parameter $\beta>0$ helps strike a balance between exploitation and exploration in the \texttt{PBMORL} process.
\end{remark}

\begin{remark}
    Note that the preference score of a policy is distinct from the information of a policy, as defined in~\pref{eq:information}. This difference arises because the objective of Step 2 is to identify policies that best represent the DM's implicit preferences. By making this distinction, our approach effectively captures the nuances of preference elicitation.
\end{remark}

\begin{remark}
    In our preliminary experiments, we observed that MORL can become overly exploitative and prone to being trapped in local optima when the \texttt{policy optimization} module is solely driven by $\dot{\mathcal{W}}$. To address this issue, Steps 3 and 4 are introduced to incorporate additional exploration outside of the ROI. This approach effectively balances exploitation and exploration, ensuring a more robust optimization process
\end{remark}

\begin{remark}
    In Step 5, the composition of $\mathcal{W}$ is designed to strike a balance between exploitation and exploration, with a focus on enhancing exploitation to accelerate convergence. In practice, we set $\kappa_1=80\%\times|\Pi|$ and $\kappa_2=20\%\times|\Pi|$. We will conduct a parameter sensitivity study on the settings of $\kappa_1$ and $\kappa_2$ in~\pref{sec:rq4} of our empirical study.
\end{remark}

\vspace{-1em}
\subsection{Policy Optimization}
\label{sec:policy_optimization}

In the \texttt{policy optimization} module, we employ the \texttt{MOPPO} algorithm, as done in the \texttt{seeding} module introduced in~\pref{sec:seeding}, which utilizes the biased weight vectors generated in the \texttt{preference elicitation} module to guide the MORL process. It is important to note that the outputs of this \texttt{policy optimization} module are fed back into the \texttt{preference elicitation} module, further enhancing the navigation towards the DM's preferred non-dominated policies until the stopping criterion are met.

\subsection{Time Complexity Analysis}
\label{sec:time complexity}

Since the \texttt{seeding} and the \texttt{policy optimization} modules of \our\ are MORL based on PPO, the corresponding time complexity is bounded by the PPO itself. Therefore, here we focus on analyzing the time complexity of the \texttt{preference elicitation} module, which consists of three steps. Specifically, during the \texttt{consultation} step, the preference model first evaluate the quality of policies in $\Pi$ which incurs $\mathcal{O}(|\Pi|)$ evaluations. Then, it chooses two elite policies to query the DM. After the DM's feedback is collected, the complexity of the \texttt{preference learning} step is bounded by $\mathcal{O}(\kappa^3)$, where $\kappa$ is the number of data instances in the training set. During the \texttt{preference translation} step, the computational complexity is mainly dominated by the ranking of policies in $\Pi$, i.e., $\mathcal{O}(|\Pi|\log |\Pi|)$. All in all, the time complexity of the \texttt{preference elicitation} module is $\max\left\{\mathcal{O}(\kappa^3),\mathcal{O}(|\Pi|\log |\Pi|)\right\}$.


==> mining.tex <==
%!TeX root=main.tex

\section{Text Mining}
\label{sec:text_mining}

